The Next Generation Global Gravitational Wave Observatory: The Science Book

The next generation of ground-based gravitational-wave detectors will observe coalescences of black holes and neutron stars throughout the cosmos, thousands of them with exceptional fidelity. The Science Book is the result of a 3-year effort to study the science capabilities of networks of next generation detectors. Such networks would make it possible to address unsolved problems in numerous areas of physics and astronomy, from Cosmology to Beyond the Standard Model of particle physics, and how they could provide insights into workings of strongly gravitating systems, astrophysics of compact objects and the nature of dense matter. It is inevitable that observatories of such depth and finesse will make new discoveries inaccessible to other windows of observation. In addition to laying out the rich science potential of the next generation of detectors, this report provides specific science targets in five different areas in physics and astronomy and the sensitivity requirements to accomplish those science goals. This report is the second in a six part series of reports by the GWIC 3G Subcommittee: i) Expanding the Reach of Gravitational Wave Observatories to the Edge of the Universe, ii) The Next Generation Global Gravitational Wave Observatory: The Science Book (this report), iii) 3G R&D: R&D for the Next Generation of Ground-based Gravitational Wave Detectors, iv) Gravitational Wave Data Analysis: Computing Challenges in the 3G Era, v) Future Ground-based Gravitational-wave Observatories: Synergies with Other Scientific Communities, and vi) An Exploration of Possible Governance Models for the Future Global Gravitational-Wave Observatory Network.

==> authors-science-book.tex <==
\nolinebreak[4]
\begin{titlepage}
\title{List of Authors}
\author[1]{\small P.~Ajith }
\author[2]{\small Shreya Anand }
\author[2]{\small Igor Andreoni }
\author[3]{\small K.G.~Arun }
\author[4]{\small Matthew Bailes }
\author[5]{\small Enrico Barausse }
\author[6]{\small Masha Baryakhtar }
\author[7]{\small Enis Belgacem }
\author[8]{\small Christopher P.L. Berry }
\author[9]{\small Daniele Bertacca }
\author[10]{\small Marie-Anne Bizouard }
\author[11]{\small Richard Brito }
\author[12]{\small Alessandra Buonanno }
\author[13]{\small Adam Burrows }
\author[14]{\small Chiara Caprini }
\author[2]{\small Katerina Chatziioannou }
\author[15]{\small Monica Colpi }
\author[16]{\small Michael Coughlin }
\author[17]{\small Giulia Cusin }
\author[18]{\small Tim Dietrich }
\author[19]{\small Yves Dirian }
\author[20]{\small William East }
\author[21]{\small Matthew Evans }
\author[22]{\small Stephen Fairhurst }
\author[23]{\small Xilong Fan }
\author[24]{\small Daniel Figueroa }
\author[25]{\small Stefano Foffa }
\author[26]{\small Archisman Ghosh }
\author[27]{\small Evan Hall }
\author[28]{\small Jan Harms }
\author[29]{\small Ian Harry }
\author[30]{\small Stefan Hild }
\author[7]{\small Tanja Hinderer }
\author[31]{\small Thomas Janka }
\author[32]{\small Stephen Justham }
\author[8]{\small Vicky Kalogera }
\author[33]{\small Dan Kasen }
\author[2]{\small Mansi M. Kasliwal }
\author[34]{\small Kei Kotake }
\author[20]{\small Luis Lehner }
\author[35]{\small Geoffrey Lovelace }
\author[36]{\small Michele Maggiore }
\author[4]{\small Ilya Mandel }
\author[16]{\small Vuk Mandic }
\author[37]{\small Alberto Mangiagli }
\author[9]{\small Michela Mapelli }
\author[28]{\small Andrea Maselli }
\author[38]{\small Andrew Matas }
\author[39]{\small Jess McIver }
\author[40]{\small Bronson Messer }
\author[40]{\small Tony Mezzacappa }
\author[22]{\small Cameron Mills }
\author[4]{\small Bernhard Mueller }
\author[31]{\small Ewald Mueller }
\author[41]{\small Samaya Nissanke }
\author[38]{\small Michael P\"urrer }
\author[11]{\small Paolo Pani }
\author[42]{\small Maria Alessandra Papa }
\author[43]{\small Geraint Pratten }
\author[44]{\small Sanjay Reddy }
\author[45]{\small Tania Regimbau }
\author[46]{\small Stephan Rosswog }
\author[47]{\small Mairi Sakellariadou }
\author[48]{\small B.S. Sathyaprakash }
\author[49]{\small Raffaella Schneider }
\author[50]{\small Alberto Sesana }
\author[51]{\small Lijing Shao }
\author[52]{\small P. Thomas Sotiriou }
\author[38]{\small Nicola Tamanini }
\author[53]{\small Thomas Tauris }
\author[4]{\small Eric Thrane }
\author[49]{\small Rosa Valiante }
\author[38]{\small Maaretn van de Meent }
\author[26]{\small Chris Van Den Broeck }
\author[2]{\small Vijay Varma }
\author[38]{\small Justin Vines }
\author[27]{\small Salvatore Vitale }
\author[20]{\small Huan Yang }
\author[54]{\small Nicolas Yunes }
\author[55]{\small Miguel Zumalacarregui }

\affil[1]{\small International Centre for Theoretical Sciences, India }
\affil[2]{\small California Institute of Technology, USA }
\affil[3]{\small Chennai Mathematical Institute, India }
\affil[4]{\small OzGrav, Centre for Astrophysics and Supercomputing, Swinburne University, Australia }
\affil[5]{\small Institut d'Astrophysique de Paris, France }
\affil[6]{\small New York University, USA }
\affil[7]{\small Utrecht University, The Netherlands }
\affil[8]{\small Northwestern University, USA }
\affil[9]{\small Universit\'a degli Studi di Padova, Italy and INFN Sezione di Padova, Italy }
\affil[10]{\small Artemis, CNRS \& Observatoire de la Cote d'Azur, France }
\affil[11]{\small Sapienza University of Rome, Italy }
\affil[12]{\small Max Planck Institute for Gravitational Physics, Potsdam, Germany and University of Maryland, USA }
\affil[13]{\small Princeton University, USA }
\affil[14]{\small Universit\'e Paris-Diderot, France }
\affil[15]{\small University of Milano -- Bicocca, Italy }
\affil[16]{\small University of Minnesota, USA }
\affil[17]{\small University of Oxford, United Kingdom }
\affil[18]{\small University of Potsdam, Germany }
\affil[19]{\small University of Geneva and University of Zuerich, Switzerland }
\affil[20]{\small Perimeter Institute, Canada }
\affil[21]{\small Massachusetts Institute of Technology, USA }
\affil[22]{\small Cardiff University, UK }
\affil[23]{\small Wuhan University and Hubei University of Education, China }
\affil[24]{\small \'Ecole Polytechnique F\'ed\'erale de Lausanne, Switzerland }
\affil[25]{\small University of Geneva, Switzerland }
\affil[26]{\small Nikhef, The Netherlands }
\affil[27]{\small Massachusetts Institute of Technology, USA }
\affil[28]{\small Gran Sasso Science Institute, Italy }
\affil[29]{\small Max Planck Institute for Gravitational Physics, Potsdam, Germany and University of Portsmouth, UK }
\affil[30]{\small Mastricht University, The Netherlands }
\affil[31]{\small Max Planck Institute for Astrophysics, Germany }
\affil[32]{\small UCAS, China and University of Amsterdam, Holland }
\affil[33]{\small University of California Berkeley, USA }
\affil[34]{\small Fukuoka University, Japan }
\affil[35]{\small California State University Fullerton, USA }
\affil[36]{\small University of Geneva, Switzerland }
\affil[37]{\small Astroparticule et Cosmologie, France }
\affil[38]{\small Max Planck Institute for Gravitational Physics, Potsdam, Germany }
\affil[39]{\small Caltech, USA and the University of British Columbia, Canada }
\affil[40]{\small ORNL and University of Tennessee, USA }
\affil[41]{\small University of Amsterdam, The Netherlands }
\affil[42]{\small Max Planck Institute for Gravitational Physics, Hannover, Germany and University of Wisconsin, Milwaukee, USA }
\affil[43]{\small University of Balearic Islands, Spain and University of Birmingham, UK }
\affil[44]{\small Institute for Nuclear Theory, University of Washington, Seattle, USA }
\affil[45]{\small Universit\'e Grenoble Alpes, France }
\affil[46]{\small Stockholms University, Sweden }
\affil[47]{\small Kings College London, United Kingdom }
\affil[48]{\small Penn State University, USA and Cardiff University, UK }
\affil[49]{\small INFN Roma, Italy }
\affil[50]{\small Universita` di Milano-Bicocca, Italy }
\affil[51]{\small Kavli Institute for Astronomy and Astrophysics, Peking University, China }
\affil[52]{\small The University of Nottingham, UK }
\affil[53]{\small Aarhus University, Greece }
\affil[54]{\small Montana State University, USA }
\affil[55]{\small University of California Berkely, USA and IPhT, Saclay, France }
\date{}

%\let\original\newpage
%\let\newpage\relax
\maketitle
%\let\newpage\original
\end{titlepage}
